ActiveDP: Bridging Active Learning and Data Programming

Modern machine learning models require large labelled datasets to achieve good performance, but manually labelling large datasets is expensive and time-consuming. The data programming paradigm enables users to label large datasets efficiently but produces noisy labels, which deteriorates the downstream model's performance. The active learning paradigm, on the other hand, can acquire accurate labels but only for a small fraction of instances. In this paper, we propose ActiveDP, an interactive framework bridging active learning and data programming together to generate labels with both high accuracy and coverage, combining the strengths of both paradigms. Experiments show that ActiveDP outperforms previous weak supervision and active learning approaches and consistently performs well under different labelling budgets.

==> 02_preliminary.tex <==
\section{Preliminaries} \label{sec:preliminary}
In this section, we review the DP paradigm \cite{ratner2017snorkel}, the IDP paradigm \cite{hsieh2022nemo}, and active learning \cite{settles2009active}. Let each instance $x\in X$ be coupled with a class label $y\in Y$, where the underlying joint distribution is $P$. Given a dataset $D=\{x_i\}_{i=1}^n$ drawn from $P$ with unobserved labels, the data programming paradigm automatically labels the dataset for model training with the following three stages:
\begin{enumerate}

\item Label Function Design: The users design a set of label functions (LFs) $\{\lambda_j\}_{j=1}^m$, which are rules that provide noisy labels to a subset of data. When a label function $\lambda_j$ takes an instance $x_i $ as input, it either labels it with $\lambda_j(x_i)\in Y$ or abstains with $\lambda_j(x_i)= -1$. The outputs of label functions are called weak labels. 

\item Label Model Training: By applying the m label functions on n instances, we get a label matrix $\Lambda(D)\in R^{n*m}$ consisting of all weak labels. Then a label model $f_l$ takes the label matrix as input and learns to denoise the conflicting weak labels. The label model would produce a single probabilistic label for each instance, denoted as $\hat{y}_i = f_l (\Lambda, x_i)$. 

\item End Model Training: The probabilistic labels will be used to create a labelled dataset $(x_i, \hat{y}_i)_{i=1}^n$ for training the downstream model $f_e$. The goal is to minimize the generation error of the downstream model on distribution $P$.

\end{enumerate}

As human experts often refer to some development data sampled from the unlabeled dataset to help LF design, the interactive data programming (IDP) paradigm \cite{hsieh2022nemo} formalizes LF design as an interactive process and guides human experts by strategically selecting the development data. At each iteration, the system picks a subset of examples $S_t\in D$ for human experts to check. The human experts then design a set of label functions $\Lambda_t=\{\lambda_{t_1},...,\lambda_{t_k}\}$ based on $S_t$. When the interactive process terminates, the label model and end model are learned from  $\{(\Lambda_1,S_1),...,(\Lambda_t,S_t)\}$, with $\Lambda=\Lambda_1\cup ...\cup \Lambda_t$ being the final LF set and $\{S_1,...,S_t\}$ being used to prevent LF over-generalization.

Instead of labelling the vast dataset, the active learning paradigm \cite{settles2009active} iteratively selects a subset of data instances $\{x_{l_t}\}_{t=1}^T$ for manual labelling and uses the labelled subset to train an active learning model $f_a$ instead. The instances are carefully selected to be diverse and informative to improve the performance of the active learning model. We discuss more selection strategies in Section \ref{sec:background}.

==> table/baseline.tex <==
\begin{table}[htbp]
\footnotesize
\centering
\caption{Performance comparison with baseline methods.}\label{tab:baseline}
\vspace{-0.1cm}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\toprule[1.5pt]
\textbf{Dataset} & \textbf{ActiveDP} & \textbf{Nemo} & \textbf{IWS} & \textbf{US} \\
\hline
Youtube & 0.8739 & 0.7628 & 0.6510 & 0.8266 \\
\hline
IMDB & 0.7988 & 0.7681 & 0.7198 & 0.6889 \\
\hline
Yelp & 0.7645 & 0.7500 & 0.5228 & 0.7255 \\
\hline
Amazon & 0.7193 & 0.7200 & 0.6769 & 0.6347 \\
\hline
Bios-prof-teach & 0.8700 & 0.8307 & 0.7298 & 0.8063 \\
\hline
Bios-jour-photo & 0.9073 & 0.8862 & 0.8631 & 0.8086 \\
\bottomrule[1.5pt]
\end{tabular}}
\end{table}

==> table/lf-acc.tex <==
\begin{table}[htbp]
\footnotesize
\centering
\caption{Performance of ActiveDP with different simulated LF accuracy thresholds.}\label{tab:lf-acc}
\vspace{-0.1cm}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c c c c c c c c c}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{LF Accuracy}} & \multicolumn{6}{c}{\textbf{Dataset}} \\
\cline{2-9}
& \textbf{Youtube} & \textbf{IMDB} & \textbf{Yelp} & \textbf{Amazon} & \textbf{Bios-PT} & \textbf{Bios-JP} & \textbf{Occupancy} & \textbf{Census} \\
\hline
0.5 & 0.8719 & 0.7232 & 0.7450 & 0.6579 & 0.8698 & 0.8944 & 0.9904 & 0.7992 \\

0.6 & 0.8894 & 0.8016 & 0.7834 & 0.7198 & 0.8785 & 0.9078 & 0.9905 & 0.8096\\

0.7 & 0.8719 & 0.7883 & 0.8083 & 0.7653 & 0.8584 & 0.9128 & 0.9922 & 0.8018\\
\bottomrule[1.5pt]
\end{tabular}}
\end{table}

==> table/lf-selector_1.tex <==
\begin{table}[htbp]
\footnotesize
\centering
\caption{Performance of ActiveDP with different Feature Selection Methods.}\label{tab:lf-selector}
\vspace{-0.1cm}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c c c c c c c}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Feature Selector}} & \multicolumn{6}{c}{\textbf{Dataset}} \\
\cline{2-7}
& \textbf{Youtube} & \textbf{IMDB} & \textbf{Yelp} & \textbf{Amazon} & \textbf{Bios-PT} & \textbf{Bios-JP} \\
\hline
LinearSVR & 0.8759 & 0.7957 & 0.7578 & 0.7122 & 0.8728 & 0.8980 \\
DT & 0.8760 & 0.7957 & 0.7567 & 0.7122 & 0.8773 & 0.8980 \\
ARD & 0.8604 & 0.7956 & 0.7572 & 0.7121 & 0.8744 & 0.8992 \\
Glasso & 0.8743 & 0.7852 & 0.7645 & 0.7193 & 0.8707 & 0.9076 \\
\bottomrule[1.5pt]
\end{tabular}}
\end{table}
